Quantum state preparation of topological chiral spin liquids via Floquet engineering

In condensed matter, Chiral Spin Liquids (CSL) are quantum spin analogs of electronic Fractional Quantum Hall states (in the continuum) or Fractional Chern Insulators (on the lattice). As the latter, CSL are remarquable states of matter, exhibiting topological order and chiral edge modes. Preparing CSL on quantum simulators like cold atom platforms is still an open challenge. Here we propose a simple setup on a finite cluster of spin-1/2 located at the sites of a square lattice. Using a Resonating Valence Bond (RVB) non-chiral spin liquid as initial state on which fast time-modulations of strong nearest-neighbor Heisenberg couplings are applied, following different protocols (out-of-equilibrium quench or semi-adiabatic ramping of the drive), we show the slow emergence of such a CSL phase. An effective Floquet dynamics, obtained from a high-frequency Magnus expansion of the drive Hamiltonian, provides a very accurate and simple framework fully capturing the out-of-equilibrium dynamics. An analysis of the resulting prepared states in term of Projected Entangled Pair states gives further insights on the topological nature of the chiral phase. Finally, we discuss possible applications to quantum computing.

==> preamble.tex <==
\usepackage{graphicx}
\usepackage{graphics}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{dsfont}
\usepackage{braket}
\usepackage{color}
\usepackage{braket,slashed}
\usepackage[mathscr]{euscript}
\definecolor{darkblue}{rgb}{0, 0, 0.8}
\usepackage[colorlinks=true, breaklinks=true, linkcolor=red, citecolor=blue, urlcolor=blue]{hyperref} 
%\usepackage{hyperref}
\usepackage{subfigure}
\usepackage{xfrac}
\usepackage{bm}
\usepackage{kantlipsum}
\usepackage{enumitem}
\usepackage{tikz}
\usepackage{framed}
\usepackage{graphicx}
\usepackage{subfigure}
%\usepackage{times}
\usepackage{cleveref}
\usepackage{adjustbox}


\usepackage{xcolor}

%\usepackage{geometry}
%\geometry{a4paper}
%\geometry{hmargin=2cm,vmargin=3cm}

\allowdisplaybreaks[1]

% code fonts
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\codestring}[1]{\code{\textquotesingle{}{#1}\textquotesingle{}}}
\newenvironment{partcode}{\begin{quote}\ttfamily}{\end{quote}}

\newenvironment{codeF}[1]{\begin{framed} \begin{quote} \par\code{#1} \vspace{\baselineskip} \par} {\end{quote} \end{framed}}

\newcommand{\functiond}[2]{ \begin{framed} \begin{quote} \par\code{#1} \vspace{\baselineskip} \par #2\end{quote} \end{framed}}

%\newenvironment{allintypewriter}{\ttfamily}{\par}

% symmetroes
\newcommand{\threej}[6]{\ensuremath{\begin{pmatrix} #1 & #2 & #3 \\ #4 & #5 & #6 \end{pmatrix}}}


% Special math fonts and notations
\newcommand{\T}{\ensuremath{\mathcal{T}}}
\newcommand{\h}[1]{\ensuremath{\hat{#1}}}
\renewcommand{\t}[1]{\ensuremath{\tilde{#1}}}
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\CC}{\ensuremath{\mathbb{C}}}
\newcommand{\voperator}[1]{\ensuremath{\breve{#1}}}
\newcommand{\manifold}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\group}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\vectorspace}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\algebra}[1]{\ensuremath{\mathfrak{#1}}}
\newcommand{\bM}{\ensuremath{{\bar{M}}}}

% Math operators
\DeclareMathOperator*{\varmin}{min}
\DeclareMathOperator*{\varmax}{max}
\DeclareMathOperator*{\argmin}{arg\ min}
\DeclareMathOperator*{\argmax}{arg\ max}
\DeclareMathOperator{\order}{\mathscr{O}}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\sign}{sgn}
\DeclareMathOperator{\End}{\mathbb{L}}
\DeclareMathOperator{\spanop}{span}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\arccosh}{arccosh}
\DeclareMathOperator{\arcsinh}{arcsinh}

\newcommand{\commutator}[2]{\ensuremath{\left[#1,#2\right]}}
\newcommand{\anticommutator}[2]{\ensuremath{\left\{#1,#2\right\}}}
\newcommand{\sgn}{\ensuremath{\text{sgn}}}
\newcommand{\Pv}{\ensuremath{\text{Pv}\,}}



\newcommand{\one}{\mathds{1}}
\newcommand{\zero}{\mathds{0}}
\renewcommand{\dag}{^\dagger}
\newcommand{\pdag}{^{\phantom{\dagger}}}
\newcommand{\up}{{\uparrow}}
\renewcommand{\do}{\downarrow}
\newcommand{\updo}{{\uparrow\downarrow}}
\renewcommand{\d}{\ensuremath{\mathrm{d}}}
\newcommand{\e}{\ensuremath{\mathrm{e}}}
\newcommand{\grad}{\ensuremath{\vec{\nabla}}}
\newcommand{\ham}{\ensuremath{\hat{H}}}
\newcommand{\ovr}{\ensuremath{\overline{\bm{r}}}}
\newcommand{\orr}{\ensuremath{\overline{r}}}
\newcommand{\ic}{\ensuremath{i}}

\newcommand{\SU}{\ensuremath{\mathrm{SU}}}
\newcommand{\He}{\ensuremath{H_{\mathrm{ent}}}}
\newcommand{\vS}{\ensuremath{\vec{S}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\U}{\ensuremath{\mathrm{U}}}

\newcommand{\rket}[1]{\ensuremath{|#1)}}
\newcommand{\rbra}[1]{\ensuremath{(#1|}}
\newcommand{\rbraket}[1]{\ensuremath{(#1)}}
\newcommand{\Rket}[1]{\ensuremath{\left|#1\right)}}
\newcommand{\Rbra}[1]{\ensuremath{\left(#1\right|}}
\newcommand{\Rbraket}[1]{\ensuremath{\left(#1\right)}}

\newcommand{\vect}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\spst}{\ensuremath{\ket{\{s\}}}}
\newcommand{\E}[2]{\ensuremath{E^{#1}_{#2}}}
\renewcommand{\O}[2]{\ensuremath{O^{#1}_{#2}}}
\renewcommand{\H}[4]{\ensuremath{H^{#1#2}_{#3#4}}}
\newcommand{\I}[6]{\ensuremath{I^{#1#2#3}_{#4#5#6}}}
\newcommand{\HH}[6]{\ensuremath{H^{#1#2#3}_{#4#5#6}}}
\newcommand{\J}[4]{\ensuremath{J^{#1#2}_{#3#4}}}
\newcommand{\tA}{\ensuremath{A}}
\newcommand{\alphap}{\ensuremath{{\alpha'}}}
\newcommand{\betap}{\ensuremath{{\beta'}}}
\newcommand{\gammap}{\ensuremath{{\gamma'}}}
\newcommand{\perm}{\ensuremath{{\mathcal{P}}}}
\newcommand{\vv}{\ensuremath{\vect{v}}}
\newcommand{\Tr}{\ensuremath{\text{Tr}}}

\newcommand{\diagram}[1]{\;\vcenter{\hbox{\includegraphics[scale=0.32,page=#1]{./Figures/diagrams.pdf}}}\;}
\newcommand{\tmdiags}[2]{\;\vcenter{\hbox{\includegraphics[scale=#2,page=#1]{./Figures/tmdiags.pdf}}}\;}

\newcommand{\pepo}[1]{\;\vcenter{\hbox{\includegraphics{#1}}}\;}
\newcommand{\pepob}[2]{\;\vcenter{\hbox{\includegraphics[scale=#2]{#1}}}\;}

\newcommand{\lv}[1]{{\color{blue} #1}}
